Engineering of a Low-Entropy Quantum Simulator for Strongly Correlated Electrons Using SU($\mathcal{N}$)-Symmetric Cold Atom Mixtures

An advanced cooling scheme, incorporating entropy engineering, is vital for isolated artificial quantum systems designed to emulate the low-temperature physics of strongly correlated electron systems (SCESs). This study theoretically demonstrates a cooling method employing multi-component Fermi gases with SU($\mathcal{N}$)-symmetric interactions, focusing on the case of $^{173}$Yb atoms in a two-dimensional optical lattice. Adiabatically introducing a nonuniform state-selective laser gives rise to two distinct subsystems: a central low-temperature region, exclusively composed of two specific spin components, acts as a quantum simulator for SCESs, while the surrounding $\mathcal{N}$-component mixture retains a significant portion of the entropy of the system. The SU($\mathcal{N}$)-symmetric interactions ensure that the total particle numbers for each component become good quantum numbers, creating a sharp boundary for the two-component region. The cooling efficiency is assessed through extensive finite-temperature Lanczos calculations. The results lay the foundation for quantum simulations of two-dimensional systems of Hubbard or Heisenberg type, offering crucial insights into intriguing low-temperature phenomena in condensed-matter physics.

==> bibold.tex <==
@PREAMBLE{
 "\providecommand{\noopsort}[1]{}" 
 # "\providecommand{\singleletter}[1]{#1}%" 
}

@article{Bloch2005,
  doi = {10.1038/nphys138},
  url = {https://doi.org/10.1038/nphys138},
  year = {2005},
  month = oct,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {1},
  number = {1},
  pages = {23--30},
  author = {Immanuel Bloch},
  title = {Ultracold quantum gases in optical lattices},
  journal = {Nat. Phys.}
}

@article{Bloch2012,
  doi = {10.1038/nphys2259},
  url = {https://doi.org/10.1038/nphys2259},
  year = {2012},
  month = apr,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {8},
  number = {4},
  pages = {267--276},
  author = {Immanuel Bloch and Jean Dalibard and Sylvain Nascimb{\`{e}}ne},
  title = {Quantum simulations with ultracold quantum gases},
  journal = {Nat. Phys.}
}

@article{Gross2017,
  doi = {10.1126/science.aal3837},
  url = {https://doi.org/10.1126/science.aal3837},
  year = {2017},
  month = sep,
  publisher = {American Association for the Advancement of Science ({AAAS})},
  volume = {357},
  number = {6355},
  pages = {995--1001},
  author = {Christian Gross and Immanuel Bloch},
  title = {Quantum simulations with ultracold atoms in optical lattices},
  journal = {Science}
}

@article{TAKAHASHI2022,
  doi = {10.2183/pjab.98.010},
  url = {https://doi.org/10.2183/pjab.98.010},
  year = {2022},
  month = apr,
  publisher = {Japan Academy},
  volume = {98},
  number = {4},
  pages = {141--160},
  author = {Yoshiro Takahashi},
  title = {Quantum simulation of quantum many-body systems with ultracold two-electron atoms in an optical lattice},
  journal = {Proceedings of the Japan Academy, Series B}
}

@article{Zhang2014,
  doi = {10.1126/science.1254978},
  url = {https://doi.org/10.1126/science.1254978},
  year = {2014},
  month = sep,
  publisher = {American Association for the Advancement of Science ({AAAS})},
  volume = {345},
  number = {6203},
  pages = {1467--1473},
  author = {X. Zhang and M. Bishof and S. L. Bromley and C. V. Kraus and M. S. Safronova and P. Zoller and A. M. Rey and J. Ye},
  title = {Spectroscopic observation of {SU}(
		            $\less$i$\greater$N$\less$/i$\greater$
		            )-symmetric interactions in Sr orbital magnetism},
  journal = {Science}
}

@article{Browaeys2020,
  doi = {10.1038/s41567-019-0733-z},
  url = {https://doi.org/10.1038/s41567-019-0733-z},
  year = {2020},
  month = jan,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {16},
  number = {2},
  pages = {132--142},
  author = {Antoine Browaeys and Thierry Lahaye},
  title = {Many-body physics with individually controlled Rydberg atoms},
  journal = {Nat. Phys.}
}

@article{Nogrette2014,
  doi = {10.1103/physrevx.4.021034},
  url = {https://doi.org/10.1103/physrevx.4.021034},
  year = {2014},
  month = may,
  publisher = {American Physical Society ({APS})},
  volume = {4},
  number = {2},
  pages = {021034},
  author = {F. Nogrette and H. Labuhn and S. Ravets and D. Barredo and L. B{\'{e}}guin and A. Vernier and T. Lahaye and A. Browaeys},
  title = {Single-Atom Trapping in Holographic 2D Arrays of Microtraps with Arbitrary Geometries},
  journal = {Physical Review X}
}

@article{Bernien2017,
  doi = {10.1038/nature24622},
  url = {https://doi.org/10.1038/nature24622},
  year = {2017},
  month = nov,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {551},
  number = {7682},
  pages = {579--584},
  author = {Hannes Bernien and Sylvain Schwartz and Alexander Keesling and Harry Levine and Ahmed Omran and Hannes Pichler and Soonwon Choi and Alexander S. Zibrov and Manuel Endres and Markus Greiner and Vladan Vuleti{\'{c}} and Mikhail D. Lukin},
  title = {Probing many-body dynamics on a 51-atom quantum simulator},
  journal = {Nature}
}


@article{Scholl2021,
  doi = {10.1038/s41586-021-03585-1},
  url = {https://doi.org/10.1038/s41586-021-03585-1},
  year = {2021},
  month = jul,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {595},
  number = {7866},
  pages = {233--238},
  author = {Pascal Scholl and Michael Schuler and Hannah J. Williams and Alexander A. Eberharter and Daniel Barredo and Kai-Niklas Schymik and Vincent Lienhard and Louis-Paul Henry and Thomas C. Lang and Thierry Lahaye and Andreas M. L\"{a}uchli and Antoine Browaeys},
  title = {Quantum simulation of 2D antiferromagnets with hundreds of Rydberg atoms},
  journal = {Nature}
}

@article{Ebadi2021,
  doi = {10.1038/s41586-021-03582-4},
  url = {https://doi.org/10.1038/s41586-021-03582-4},
  year = {2021},
  month = jul,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {595},
  number = {7866},
  pages = {227--232},
  author = {Sepehr Ebadi and Tout T. Wang and Harry Levine and Alexander Keesling and Giulia Semeghini and Ahmed Omran and Dolev Bluvstein and Rhine Samajdar and Hannes Pichler and Wen Wei Ho and Soonwon Choi and Subir Sachdev and Markus Greiner and Vladan Vuleti{\'{c}} and Mikhail D. Lukin},
  title = {Quantum phases of matter on a 256-atom programmable quantum simulator},
  journal = {Nature}
}

@article{Blatt2012,
  doi = {10.1038/nphys2252},
  url = {https://doi.org/10.1038/nphys2252},
  year = {2012},
  month = apr,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {8},
  number = {4},
  pages = {277--284},
  author = {R. Blatt and C. F. Roos},
  title = {Quantum simulations with trapped ions},
  journal = {Nat. Phys.}
}

@article{Monroe2021,
  doi = {10.1103/revmodphys.93.025001},
  url = {https://doi.org/10.1103/revmodphys.93.025001},
  year = {2021},
  month = apr,
  publisher = {American Physical Society ({APS})},
  volume = {93},
  number = {2},
  pages = {025001},
  author = {C. Monroe and W.{\hspace{0.167em}}C. Campbell and L.-M. Duan and Z.-X. Gong and A.{\hspace{0.167em}}V. Gorshkov and P.{\hspace{0.167em}}W. Hess and R. Islam and K. Kim and N.{\hspace{0.167em}}M. Linke and G. Pagano and P. Richerme and C. Senko and N.{\hspace{0.167em}}Y. Yao},
  title = {Programmable quantum simulations of spin systems with trapped ions},
  journal = {Reviews of Modern Physics}
}

@article{AspuruGuzik2012,
  doi = {10.1038/nphys2253},
  url = {https://doi.org/10.1038/nphys2253},
  year = {2012},
  month = apr,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {8},
  number = {4},
  pages = {285--291},
  author = {Al{\'{a}}n Aspuru-Guzik and Philip Walther},
  title = {Photonic quantum simulators},
  journal = {Nat. Phys.}
}

@article{Noh2016,
  doi = {10.1088/0034-4885/80/1/016401},
  url = {https://doi.org/10.1088/0034-4885/80/1/016401},
  year = {2016},
  month = nov,
  publisher = {{IOP} Publishing},
  volume = {80},
  number = {1},
  pages = {016401},
  author = {Changsuk Noh and Dimitris G Angelakis},
  title = {Quantum simulations and many-body physics with light},
  journal = {Reports on Progress in Physics}
}

@article{Hensgens2017,
  doi = {10.1038/nature23022},
  url = {https://doi.org/10.1038/nature23022},
  year = {2017},
  month = aug,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {548},
  number = {7665},
  pages = {70--73},
  author = {T. Hensgens and T. Fujita and L. Janssen and Xiao Li and C. J. Van Diepen and C. Reichl and W. Wegscheider and S. Das Sarma and L. M. K. Vandersypen},
  title = {Quantum simulation of a Fermi{\textendash}Hubbard model using a semiconductor quantum dot array},
  journal = {Nature}
}

@article{Houck2012,
  doi = {10.1038/nphys2251},
  url = {https://doi.org/10.1038/nphys2251},
  year = {2012},
  month = apr,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {8},
  number = {4},
  pages = {292--299},
  author = {Andrew A. Houck and Hakan E. T\"{u}reci and Jens Koch},
  title = {On-chip quantum simulation with superconducting circuits},
  journal = {Nat. Phys.}
}

@article{Cirac2012,
  doi = {10.1038/nphys2275},
  url = {https://doi.org/10.1038/nphys2275},
  year = {2012},
  month = apr,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {8},
  number = {4},
  pages = {264--266},
  author = {J. Ignacio Cirac and Peter Zoller},
  title = {Goals and opportunities in quantum simulation},
  journal = {Nat. Phys.}
}

@article{Georgescu2014,
  doi = {10.1103/revmodphys.86.153},
  url = {https://doi.org/10.1103/revmodphys.86.153},
  year = {2014},
  month = mar,
  publisher = {American Physical Society ({APS})},
  volume = {86},
  number = {1},
  pages = {153--185},
  author = {I.{\hspace{0.167em}}M. Georgescu and S. Ashhab and Franco Nori},
  title = {Quantum simulation},
  journal = {Reviews of Modern Physics}
}

@article{Hempel2018,
  doi = {10.1103/physrevx.8.031022},
  url = {https://doi.org/10.1103/physrevx.8.031022},
  year = {2018},
  month = jul,
  publisher = {American Physical Society ({APS})},
  volume = {8},
  number = {3},
  pages = {031022},
  author = {Cornelius Hempel and Christine Maier and Jonathan Romero and Jarrod McClean and Thomas Monz and Heng Shen and Petar Jurcevic and Ben P. Lanyon and Peter Love and Ryan Babbush and Al{\'{a}}n Aspuru-Guzik and Rainer Blatt and Christian F. Roos},
  title = {Quantum Chemistry Calculations on a Trapped-Ion Quantum Simulator},
  journal = {Physical Review X}
}

@article{Bauer2023,
  doi = {10.1103/prxquantum.4.027001},
  url = {https://doi.org/10.1103/prxquantum.4.027001},
  year = {2023},
  month = may,
  publisher = {American Physical Society ({APS})},
  volume = {4},
  number = {2},
  pages = {027001},
  author = {Christian W. Bauer and Zohreh Davoudi and A. Baha Balantekin and Tanmoy Bhattacharya and Marcela Carena and Wibe A. de Jong and Patrick Draper and Aida El-Khadra and Nate Gemelke and Masanori Hanada and Dmitri Kharzeev and Henry Lamm and Ying-Ying Li and Junyu Liu and Mikhail Lukin and Yannick Meurice and Christopher Monroe and Benjamin Nachman and Guido Pagano and John Preskill and Enrico Rinaldi and Alessandro Roggero and David I. Santiago and Martin J. Savage and Irfan Siddiqi and George Siopsis and David Van Zanten and Nathan Wiebe and Yukari Yamauchi and K\"{u}bra Yeter-Aydeniz and Silvia Zorzetti},
  title = {Quantum Simulation for High-Energy Physics},
  journal = {{PRX} Quantum}
}

@article{Altman2021,
  doi = {10.1103/prxquantum.2.017003},
  url = {https://doi.org/10.1103/prxquantum.2.017003},
  year = {2021},
  month = feb,
  publisher = {American Physical Society ({APS})},
  volume = {2},
  number = {1},
  pages = {017003},
  author = {Ehud Altman and Kenneth R. Brown and Giuseppe Carleo and Lincoln D. Carr and Eugene Demler and Cheng Chin and Brian DeMarco and Sophia E. Economou and Mark A. Eriksson and Kai-Mei C. Fu and Markus Greiner and Kaden R.A. Hazzard and Randall G. Hulet and Alicia J. Koll{\'{a}}r and Benjamin L. Lev and Mikhail D. Lukin and Ruichao Ma and Xiao Mi and Shashank Misra and Christopher Monroe and Kater Murch and Zaira Nazario and Kang-Kuen Ni and Andrew C. Potter and Pedram Roushan and Mark Saffman and Monika Schleier-Smith and Irfan Siddiqi and Raymond Simmonds and Meenakshi Singh and I.B. Spielman and Kristan Temme and David S. Weiss and Jelena Vu{\v{c}}kovi{\'{c}} and Vladan Vuleti{\'{c}} and Jun Ye and Martin Zwierlein},
  title = {Quantum Simulators: Architectures and Opportunities},
  journal = {{PRX} Quantum}
}

@article{Lewenstein2007,
  doi = {10.1080/00018730701223200},
  url = {https://doi.org/10.1080/00018730701223200},
  year = {2007},
  month = mar,
  publisher = {Informa {UK} Limited},
  volume = {56},
  number = {2},
  pages = {243--379},
  author = {Maciej Lewenstein and Anna Sanpera and Veronica Ahufinger and Bogdan Damski and Aditi Sen(De) and Ujjwal Sen},
  title = {Ultracold atomic gases in optical lattices: mimicking condensed matter physics and beyond},
  journal = {Advances in Physics}
}

@article{Hofstetter2018,
  doi = {10.1088/1361-6455/aaa31b},
  url = {https://doi.org/10.1088/1361-6455/aaa31b},
  year = {2018},
  month = mar,
  publisher = {{IOP} Publishing},
  volume = {51},
  number = {8},
  pages = {082001},
  author = {W Hofstetter and T Qin},
  title = {Quantum simulation of strongly correlated condensed matter systems},
  journal = {Journal of Physics B: Atomic,  Molecular and Optical Physics}
}

@incollection{Zhang2000,
  doi = {10.1007/978-3-642-59689-6_4},
  url = {https://doi.org/10.1007/978-3-642-59689-6_4},
  year = {2000},
  publisher = {Springer Berlin Heidelberg},
  pages = {37--52},
  author = {S. Zhang and E. C. Allman},
  title = {Quantum Simulations of Strongly Correlated Electron Systems},
  booktitle = {Springer Proceedings in Physics}
}

@article{Lee2006,
  doi = {10.1103/revmodphys.78.17},
  url = {https://doi.org/10.1103/revmodphys.78.17},
  year = {2006},
  month = jan,
  publisher = {American Physical Society ({APS})},
  volume = {78},
  number = {1},
  pages = {17--85},
  author = {Patrick A. Lee and Naoto Nagaosa and Xiao-Gang Wen},
  title = {Doping a Mott insulator: Physics of high-temperature superconductivity},
  journal = {Reviews of Modern Physics}
}

@book{Auerbach1994,
  doi = {10.1007/978-1-4612-0869-3},
  url = {https://doi.org/10.1007/978-1-4612-0869-3},
  year = {1994},
  publisher = {Springer New York},
  author = {Assa Auerbach},
  title = {Interacting Electrons and Quantum Magnetism}
}

@article{Moessner2006,
  doi = {10.1063/1.2186278},
  url = {https://doi.org/10.1063/1.2186278},
  year = {2006},
  month = feb,
  publisher = {{AIP} Publishing},
  volume = {59},
  number = {2},
  pages = {24--29},
  author = {Roderich Moessner and Arthur P. Ramirez},
  title = {Geometrical frustration},
  journal = {Physics Today}
}

@article{Kouwenhoven2001,
  doi = {10.1088/2058-7058/14/1/28},
  url = {https://doi.org/10.1088/2058-7058/14/1/28},
  year = {2001},
  month = jan,
  publisher = {{IOP} Publishing},
  volume = {14},
  number = {1},
  pages = {33--38},
  author = {Leo Kouwenhoven and Leonid Glazman},
  title = {Revival of the Kondo effect},
  journal = {Physics World}
}

@article{Jrdens2008,
  doi = {10.1038/nature07244},
  url = {https://doi.org/10.1038/nature07244},
  year = {2008},
  month = sep,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {455},
  number = {7210},
  pages = {204--207},
  author = {Robert J\"{o}rdens and Niels Strohmaier and Kenneth G\"{u}nter and Henning Moritz and Tilman Esslinger},
  title = {A Mott insulator of fermionic atoms in an optical lattice},
  journal = {Nature}
}

@article{Schneider2008,
  doi = {10.1126/science.1165449},
  url = {https://doi.org/10.1126/science.1165449},
  year = {2008},
  month = dec,
  publisher = {American Association for the Advancement of Science ({AAAS})},
  volume = {322},
  number = {5907},
  pages = {1520--1525},
  author = {U. Schneider and L. Hackermüller and S. Will and Th. Best and I. Bloch and T. A. Costi and R. W. Helmes and D. Rasch and A. Rosch},
  title = {Metallic and Insulating Phases of Repulsively Interacting Fermions in a 3D Optical Lattice},
  journal = {Science}
}

@article{Esslinger2010,
  doi = {10.1146/annurev-conmatphys-070909-104059},
  url = {https://doi.org/10.1146/annurev-conmatphys-070909-104059},
  year = {2010},
  month = aug,
  publisher = {Annual Reviews},
  volume = {1},
  number = {1},
  pages = {129--152},
  author = {Tilman Esslinger},
  title = {Fermi-Hubbard Physics with Atoms in an Optical Lattice},
  journal = {Annual Review of Condensed Matter Physics}
}

@article{Greif2013,
  doi = {10.1126/science.1236362},
  url = {https://doi.org/10.1126/science.1236362},
  year = {2013},
  month = jun,
  publisher = {American Association for the Advancement of Science ({AAAS})},
  volume = {340},
  number = {6138},
  pages = {1307--1310},
  author = {Daniel Greif and Thomas Uehlinger and Gregor Jotzu and Leticia Tarruell and Tilman Esslinger},
  title = {Short-Range Quantum Magnetism of Ultracold Fermions in an Optical Lattice},
  journal = {Science}
}

@article{Duarte2015,
  doi = {10.1103/physrevlett.114.070403},
  url = {https://doi.org/10.1103/physrevlett.114.070403},
  year = {2015},
  month = feb,
  publisher = {American Physical Society ({APS})},
  volume = {114},
  number = {7},
  pages = {070403},
  author = {Pedro M. Duarte and Russell A. Hart and Tsung-Lin Yang and Xinxing Liu and Thereza Paiva and Ehsan Khatami and Richard T. Scalettar and Nandini Trivedi and Randall G. Hulet},
  title = {Compressibility of a Fermionic Mott Insulator of Ultracold Atoms},
  journal = {Physical Review Letters}
}

@article{Hart2015,
  doi = {10.1038/nature14223},
  url = {https://doi.org/10.1038/nature14223},
  year = {2015},
  month = feb,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {519},
  number = {7542},
  pages = {211--214},
  author = {Russell A. Hart and Pedro M. Duarte and Tsung-Lin Yang and Xinxing Liu and Thereza Paiva and Ehsan Khatami and Richard T. Scalettar and Nandini Trivedi and David A. Huse and Randall G. Hulet},
  title = {Observation of antiferromagnetic correlations in the Hubbard model with ultracold atoms},
  journal = {Nature}
}

@article{Greif2016,
  doi = {10.1126/science.aad9041},
  url = {https://doi.org/10.1126/science.aad9041},
  year = {2016},
  month = feb,
  publisher = {American Association for the Advancement of Science ({AAAS})},
  volume = {351},
  number = {6276},
  pages = {953--957},
  author = {Daniel Greif and Maxwell F. Parsons and Anton Mazurenko and Christie S. Chiu and Sebastian Blatt and Florian Huber and Geoffrey Ji and Markus Greiner},
  title = {Site-resolved imaging of a fermionic Mott insulator},
  journal = {Science}
}

@article{Parsons2016,
  doi = {10.1126/science.aag1430},
  url = {https://doi.org/10.1126/science.aag1430},
  year = {2016},
  month = sep,
  publisher = {American Association for the Advancement of Science ({AAAS})},
  volume = {353},
  number = {6305},
  pages = {1253--1256},
  author = {Maxwell F. Parsons and Anton Mazurenko and Christie S. Chiu and Geoffrey Ji and Daniel Greif and Markus Greiner},
  title = {Site-resolved measurement of the spin-correlation function in the Fermi-Hubbard model},
  journal = {Science}
}

@article{Boll2016,
  doi = {10.1126/science.aag1635},
  url = {https://doi.org/10.1126/science.aag1635},
  year = {2016},
  month = sep,
  publisher = {American Association for the Advancement of Science ({AAAS})},
  volume = {353},
  number = {6305},
  pages = {1257--1260},
  author = {Martin Boll and Timon A. Hilker and Guillaume Salomon and Ahmed Omran and Jacopo Nespolo and Lode Pollet and Immanuel Bloch and Christian Gross},
  title = {Spin- and density-resolved microscopy of antiferromagnetic correlations in Fermi-Hubbard chains},
  journal = {Science}
}

@article{Cheuk2016sc,
  doi = {10.1126/science.aag3349},
  url = {https://doi.org/10.1126/science.aag3349},
  year = {2016},
  month = sep,
  publisher = {American Association for the Advancement of Science ({AAAS})},
  volume = {353},
  number = {6305},
  pages = {1260--1264},
  author = {Lawrence W. Cheuk and Matthew A. Nichols and Katherine R. Lawrence and Melih Okan and Hao Zhang and Ehsan Khatami and Nandini Trivedi and Thereza Paiva and Marcos Rigol and Martin W. Zwierlein},
  title = {Observation of spatial charge and spin correlations in the 2D Fermi-Hubbard model},
  journal = {Science}
}

@article{Cheuk2016,
  doi = {10.1103/physrevlett.116.235301},
  url = {https://doi.org/10.1103/physrevlett.116.235301},
  year = {2016},
  month = jun,
  publisher = {American Physical Society ({APS})},
  volume = {116},
  number = {23},
  pages = {235301},
  author = {Lawrence W. Cheuk and Matthew A. Nichols and Katherine R. Lawrence and Melih Okan and Hao Zhang and Martin W. Zwierlein},
  title = {Observation of 2D Fermionic Mott Insulators of$\less$mml:math xmlns:mml="http://www.w3.org/1998/Math/{MathML}" display="inline"$\greater$$\less$mml:mrow$\greater$$\less$mml:mmultiscripts$\greater$$\less$mml:mrow$\greater$$\less$mml:mi mathvariant="normal"$\greater$K$\less$/mml:mi$\greater$$\less$/mml:mrow$\greater$$\less$mml:mprescripts /$\greater$$\less$mml:none /$\greater$$\less$mml:mrow$\greater$$\less$mml:mn$\greater$40$\less$/mml:mn$\greater$$\less$/mml:mrow$\greater$$\less$/mml:mmultiscripts$\greater$$\less$/mml:mrow$\greater$$\less$/mml:math$\greater$with Single-Site Resolution},
  journal = {Physical Review Letters}
}

@article{Drewes2017,
  doi = {10.1103/physrevlett.118.170401},
  url = {https://doi.org/10.1103/physrevlett.118.170401},
  year = {2017},
  month = apr,
  publisher = {American Physical Society ({APS})},
  volume = {118},
  number = {17},
  pages = {170401},
  author = {J.{\hspace{0.167em}}H. Drewes and L.{\hspace{0.167em}}A. Miller and E. Cocchi and C.{\hspace{0.167em}}F. Chan and N. Wurz and M. Gall and D. Pertot and F. Brennecke and M. K\"{o}hl},
  title = {Antiferromagnetic Correlations in Two-Dimensional Fermionic Mott-Insulating and Metallic Phases},
  journal = {Physical Review Letters}
}

@article{Mazurenko2017,
  doi = {10.1038/nature22362},
  url = {https://doi.org/10.1038/nature22362},
  year = {2017},
  month = may,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {545},
  number = {7655},
  pages = {462--466},
  author = {Anton Mazurenko and Christie S. Chiu and Geoffrey Ji and Maxwell F. Parsons and M{\'{a}}rton Kan{\'{a}}sz-Nagy and Richard Schmidt and Fabian Grusdt and Eugene Demler and Daniel Greif and Markus Greiner},
  title = {A cold-atom Fermi{\textendash}Hubbard antiferromagnet},
  journal = {Nature}
}

@article{Brown2017,
  doi = {10.1126/science.aam7838},
  url = {https://doi.org/10.1126/science.aam7838},
  year = {2017},
  month = sep,
  publisher = {American Association for the Advancement of Science ({AAAS})},
  volume = {357},
  number = {6358},
  pages = {1385--1388},
  author = {Peter T. Brown and Debayan Mitra and Elmer Guardado-Sanchez and Peter Schau{\ss} and Stanimir S. Kondov and Ehsan Khatami and Thereza Paiva and Nandini Trivedi and David A. Huse and Waseem S. Bakr},
  title = {Spin-imbalance in a 2D Fermi-Hubbard system},
  journal = {Science}
}

@article{Bernier2009,
  doi = {10.1103/physreva.79.061601},
  url = {https://doi.org/10.1103/physreva.79.061601},
  year = {2009},
  month = jun,
  publisher = {American Physical Society ({APS})},
  volume = {79},
  number = {6},
  pages = {061601},
  author = {Jean-S{\'{e}}bastien Bernier and Corinna Kollath and Antoine Georges and Lorenzo De Leo and Fabrice Gerbier and Christophe Salomon and Michael K\"{o}hl},
  title = {Cooling fermionic atoms in optical lattices by shaping the confinement},
  journal = {Physical Review A}
}

@article{Savary2016,
  doi = {10.1088/0034-4885/80/1/016502},
  url = {https://doi.org/10.1088/0034-4885/80/1/016502},
  year = {2016},
  month = nov,
  publisher = {{IOP} Publishing},
  volume = {80},
  number = {1},
  pages = {016502},
  author = {Lucile Savary and Leon Balents},
  title = {Quantum spin liquids: a review},
  journal = {Reports on Progress in Physics}
}



@article{Taie2022,
  doi = {10.1038/s41567-022-01725-6},
  url = {https://doi.org/10.1038/s41567-022-01725-6},
  year = {2022},
  month = sep,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {18},
  number = {11},
  pages = {1356--1361},
  author = {Shintaro Taie and Eduardo Ibarra-Garc{\'{\i}}a-Padilla and Naoki Nishizawa and Yosuke Takasu and Yoshihito Kuno and Hao-Tian Wei and Richard T. Scalettar and Kaden R. A. Hazzard and Yoshiro Takahashi},
  title = {Observation of antiferromagnetic correlations in an ultracold {SU}(N) Hubbard model},
  journal = {Nat. Phys.}
}
@article{Fukuhara2007,
  doi = {10.1103/physrevlett.98.030401},
  url = {https://doi.org/10.1103/physrevlett.98.030401},
  year = {2007},
  month = jan,
  publisher = {American Physical Society ({APS})},
  volume = {98},
  number = {3},
  pages = {030401},
  author = {Takeshi Fukuhara and Yosuke Takasu and Mitsutaka Kumakura and Yoshiro Takahashi},
  title = {Degenerate Fermi Gases of Ytterbium},
  journal = {Physical Review Letters}
}
@article{Cazalilla2009,
  doi = {10.1088/1367-2630/11/10/103033},
  url = {https://doi.org/10.1088/1367-2630/11/10/103033},
  year = {2009},
  month = oct,
  publisher = {{IOP} Publishing},
  volume = {11},
  number = {10},
  pages = {103033},
  author = {M A Cazalilla and A F Ho and M Ueda},
  title = {Ultracold gases of ytterbium: ferromagnetism and Mott states in an {SU}(6) Fermi system},
  journal = {New Journal of Physics}
}

@article{Gorshkov2010,
  doi = {10.1038/nphys1535},
  url = {https://doi.org/10.1038/nphys1535},
  year = {2010},
  month = feb,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {6},
  number = {4},
  pages = {289--295},
  author = {A. V. Gorshkov and M. Hermele and V. Gurarie and C. Xu and P. S. Julienne and J. Ye and P. Zoller and E. Demler and M. D. Lukin and A. M. Rey},
  title = {Two-orbital S U(N) magnetism with ultracold alkaline-earth atoms},
  journal = {Nat. Phys.}
}

@article{Cazalilla2014,
  doi = {10.1088/0034-4885/77/12/124401},
  url = {https://doi.org/10.1088/0034-4885/77/12/124401},
  year = {2014},
  month = nov,
  publisher = {{IOP} Publishing},
  volume = {77},
  number = {12},
  pages = {124401},
  author = {Miguel A Cazalilla and Ana Maria Rey},
  title = {Ultracold Fermi gases with emergent {SU}($\less$b$\greater$$\less$i$\greater$N$\less$/i$\greater$$\less$/b$\greater$) symmetry},
  journal = {Reports on Progress in Physics}
}

@article{Hofrichter2016,
  doi = {10.1103/physrevx.6.021030},
  url = {https://doi.org/10.1103/physrevx.6.021030},
  year = {2016},
  month = jun,
  publisher = {American Physical Society ({APS})},
  volume = {6},
  number = {2},
  pages = {021030},
  author = {Christian Hofrichter and Luis Riegger and Francesco Scazza and Moritz H\"{o}fer and Diogo Rio Fernandes and Immanuel Bloch and Simon F\"{o}lling},
  title = {Direct Probing of the Mott Crossover in the$\less$mml:math xmlns:mml="http://www.w3.org/1998/Math/{MathML}" display="inline"$\greater$$\less$mml:mrow$\greater$$\less$mml:mi$\greater${SU}$\less$/mml:mi$\greater$$\less$mml:mo stretchy="false"$\greater$($\less$/mml:mo$\greater$$\less$mml:mi$\greater$N$\less$/mml:mi$\greater$$\less$mml:mo stretchy="false"$\greater$)$\less$/mml:mo$\greater$$\less$/mml:mrow$\greater$$\less$/mml:math$\greater$Fermi-Hubbard Model},
  journal = {Physical Review X}
}

@article{DeSalvo2010,
  doi = {10.1103/physrevlett.105.030402},
  url = {https://doi.org/10.1103/physrevlett.105.030402},
  year = {2010},
  month = jul,
  publisher = {American Physical Society ({APS})},
  volume = {105},
  number = {3},
  pages = {030402},
  author = {B. J. DeSalvo and M. Yan and P. G. Mickelson and Y. N. Martinez de Escobar and T. C. Killian},
  title = {Degenerate Fermi Gas of$\less$mml:math xmlns:mml="http://www.w3.org/1998/Math/{MathML}" display="inline"$\greater$$\less$mml:mmultiscripts$\greater$$\less$mml:mi$\greater$Sr$\less$/mml:mi$\greater$$\less$mml:mprescripts /$\greater$$\less$mml:none /$\greater$$\less$mml:mn$\greater$87$\less$/mml:mn$\greater$$\less$/mml:mmultiscripts$\greater$$\less$/mml:math$\greater$},
  journal = {Physical Review Letters}
}
@article{Tey2010,
  doi = {10.1103/physreva.82.011608},
  url = {https://doi.org/10.1103/physreva.82.011608},
  year = {2010},
  month = jul,
  publisher = {American Physical Society ({APS})},
  volume = {82},
  number = {1},
  pages = {011608},
  author = {Meng Khoon Tey and Simon Stellmer and Rudolf Grimm and Florian Schreck},
  title = {Double-degenerate Bose-Fermi mixture of strontium},
  journal = {Physical Review A}
}
@ARTICLE{Honerkamp2004-sj,
  title     = "Ultracold fermions and the {SU(N}) Hubbard model",
  author    = "Honerkamp, Carsten and Hofstetter, Walter",
  abstract  = "We investigate the fermionic SU(N) Hubbard model on the
               two-dimensional square lattice for weak to moderate interactions
               using renormalization group and mean-field methods. For the
               repulsive case U>0 at half filling and small N the dominant
               tendency is towards breaking of the SU(N) symmetry. For N>6
               staggered flux order takes over as the dominant instability, in
               agreement with the large-N limit. Away from half filling for N=3
               two flavors remain half filled by cannibalizing the third
               flavor. For U<0 and odd N a full Fermi surface coexists with a
               superconductor. These results may be relevant to future
               experiments with cold fermionic atoms in optical lattices.",
  journal   = "Phys. Rev. Lett.",
  publisher = "American Physical Society (APS)",
  volume    =  92,
  number    =  17,
  pages     = "170403",
  month     =  apr,
  year      =  2004,
  copyright = "http://link.aps.org/licenses/aps-default-license",
  language  = "en"
}


@ARTICLE{Hermele2009-fp,
  title     = "Mott insulators of ultracold fermionic alkaline Earth atoms:
               underconstrained magnetism and chiral spin liquid",
  author    = "Hermele, Michael and Gurarie, Victor and Rey, Ana Maria",
  abstract  = "We study Mott insulators of fermionic alkaline earth atoms,
               described by Heisenberg spin models with enhanced SU(N)
               symmetry. In dramatic contrast to SU(2) magnetism, more than two
               spins are required to form a singlet. On the square lattice, the
               classical ground state is highly degenerate and magnetic order
               is thus unlikely. In a large-N limit, we find a chiral spin
               liquid ground state with topological order and Abelian
               fractional statistics. We discuss its experimental detection.
               Chiral spin liquids with non-Abelian anyons may also be
               realizable with alkaline earth atoms.",
  journal   = "Phys. Rev. Lett.",
  publisher = "American Physical Society (APS)",
  volume    =  103,
  number    =  13,
  pages     = "135301",
  month     =  sep,
  year      =  2009,
  copyright = "http://link.aps.org/licenses/aps-default-license",
  language  = "en"
}

%---begin---------SU(N) exotic physics-------------
@article{Tth2010,
  doi = {10.1103/physrevlett.105.265301},
  url = {https://doi.org/10.1103/physrevlett.105.265301},
  year = {2010},
  month = dec,
  publisher = {American Physical Society ({APS})},
  volume = {105},
  number = {26},
  pages = {265301},
  author = {Tam{\'{a}}s A. T{\'{o}}th and Andreas M. L\"{a}uchli and Fr{\'{e}}d{\'{e}}ric Mila and Karlo Penc},
  title = {Three-Sublattice Ordering of the {SU}(3) Heisenberg Model of Three-Flavor Fermions on the Square and Cubic Lattices},
  journal = {Physical Review Letters}
}
@article{Bauer2012,
  doi = {10.1103/physrevb.85.125116},
  url = {https://doi.org/10.1103/physrevb.85.125116},
  year = {2012},
  month = mar,
  publisher = {American Physical Society ({APS})},
  volume = {85},
  number = {12},
  pages = {125116},
  author = {Bela Bauer and Philippe Corboz and Andreas M. L\"{a}uchli and Laura Messio and Karlo Penc and Matthias Troyer and Fr{\'{e}}d{\'{e}}ric Mila},
  title = {Three-sublattice order in the {SU}(3) Heisenberg model on the square and triangular lattice},
  journal = {Physical Review B}
}
@article{Nataf2014,
  doi = {10.1103/physrevlett.113.127204},
  url = {https://doi.org/10.1103/physrevlett.113.127204},
  year = {2014},
  month = sep,
  publisher = {American Physical Society ({APS})},
  volume = {113},
  number = {12},
  pages = {127204},
  author = {Pierre Nataf and Fr{\'{e}}d{\'{e}}ric Mila},
  title = {Exact Diagonalization of Heisenberg$\less$mml:math xmlns:mml="http://www.w3.org/1998/Math/{MathML}" display="inline"$\greater$$\less$mml:mrow$\greater$$\less$mml:mi$\greater${SU}$\less$/mml:mi$\greater$$\less$mml:mo stretchy="false"$\greater$($\less$/mml:mo$\greater$$\less$mml:mi$\greater$N$\less$/mml:mi$\greater$$\less$mml:mo stretchy="false"$\greater$)$\less$/mml:mo$\greater$$\less$/mml:mrow$\greater$$\less$/mml:math$\greater$Models},
  journal = {Physical Review Letters}
}
@article{Corboz2011,
  doi = {10.1103/physrevlett.107.215301},
  url = {https://doi.org/10.1103/physrevlett.107.215301},
  year = {2011},
  month = nov,
  publisher = {American Physical Society ({APS})},
  volume = {107},
  number = {21},
  pages = {215301},
  author = {Philippe Corboz and Andreas M. L\"{a}uchli and Karlo Penc and Matthias Troyer and Fr{\'{e}}d{\'{e}}ric Mila},
  title = {Simultaneous Dimerization and {SU}(4) Symmetry Breaking of 4-Color Fermions on the Square Lattice},
  journal = {Physical Review Letters}
}
@article{Hermele2011,
  doi = {10.1103/physrevb.84.174441},
  url = {https://doi.org/10.1103/physrevb.84.174441},
  year = {2011},
  month = nov,
  publisher = {American Physical Society ({APS})},
  volume = {84},
  number = {17},
  pages = {174441},
  author = {Michael Hermele and Victor Gurarie},
  title = {Topological liquids and valence cluster states in two-dimensional {SU}$\less$mml:math xmlns:mml="http://www.w3.org/1998/Math/{MathML}" display="inline"$\greater$$\less$mml:mrow$\greater$$\less$mml:mo$\greater$($\less$/mml:mo$\greater$$\less$mml:mi$\greater$N$\less$/mml:mi$\greater$$\less$mml:mo$\greater$)$\less$/mml:mo$\greater$$\less$/mml:mrow$\greater$$\less$/mml:math$\greater$magnets},
  journal = {Physical Review B}
}
@article{Romen2020,
  doi = {10.1103/physrevresearch.2.043009},
  url = {https://doi.org/10.1103/physrevresearch.2.043009},
  year = {2020},
  month = oct,
  publisher = {American Physical Society ({APS})},
  volume = {2},
  number = {4},
  pages = {043009},
  author = {Christian Romen and Andreas M. L\"{a}uchli},
  title = {Structure of spin correlations in high-temperature 
		$\less$mml:math xmlns:mml="http://www.w3.org/1998/Math/{MathML}"$\greater$$\less$mml:mrow$\greater$$\less$mml:mi$\greater${SU}$\less$/mml:mi$\greater$$\less$mml:mo$\greater$($\less$/mml:mo$\greater$$\less$mml:mi$\greater$N$\less$/mml:mi$\greater$$\less$mml:mo$\greater$)$\less$/mml:mo$\greater$$\less$/mml:mrow$\greater$$\less$/mml:math$\greater$
		 quantum magnets},
  journal = {Physical Review Research}
}
@article{Yamamoto2020,
  doi = {10.1103/physrevlett.125.057204},
  url = {https://doi.org/10.1103/physrevlett.125.057204},
  year = {2020},
  month = jul,
  publisher = {American Physical Society ({APS})},
  volume = {125},
  number = {5},
  pages = {057204},
  author = {Daisuke Yamamoto and Chihiro Suzuki and Giacomo Marmorini and Sho Okazaki and Nobuo Furukawa},
  title = {Quantum and Thermal Phase Transitions of the Triangular {SU}(3) Heisenberg Model under Magnetic Fields},
  journal = {Physical Review Letters}
}
@article{Motegi2023,
  doi = {10.1103/physrevresearch.5.l022056},
  url = {https://doi.org/10.1103/physrevresearch.5.l022056},
  year = {2023},
  month = jun,
  publisher = {American Physical Society ({APS})},
  volume = {5},
  number = {2},
  pages = {l022056},
  author = {Hayato Motegi and Giacomo Marmorini and Nobuo Furukawa and Daisuke Yamamoto},
  title = {Thermal Ising transition in two-dimensional {SU}(3) Fermi lattice gases with population imbalance},
  journal = {Physical Review Research}
}
@article{Miyazaki2022,
  doi = {10.7566/jpsj.91.073702},
  url = {https://doi.org/10.7566/jpsj.91.073702},
  year = {2022},
  month = jul,
  publisher = {Physical Society of Japan},
  volume = {91},
  number = {7},
  pages = {073702},
  author = {Yuki Miyazaki and Giacomo Marmorini and Nobuo Furukawa and Daisuke Yamamoto},
  title = {Linear Flavor-Wave Analysis of {SU}(4)-Symmetric Tetramer Model with Population Imbalance},
  journal = {Journal of the Physical Society of Japan}
}

%----end----------SU(N) exotic physics-------------

@article{Richardson1997,
  doi = {10.1103/revmodphys.69.683},
  url = {https://doi.org/10.1103/revmodphys.69.683},
  year = {1997},
  month = jul,
  publisher = {American Physical Society ({APS})},
  volume = {69},
  number = {3},
  pages = {683--690},
  author = {Robert C. Richardson},
  title = {The Pomeranchuk effect},
  journal = {Reviews of Modern Physics}
}

@article{ColomTatch2011,
  doi = {10.1088/1367-2630/13/11/113021},
  url = {https://doi.org/10.1088/1367-2630/13/11/113021},
  year = {2011},
  month = nov,
  publisher = {{IOP} Publishing},
  volume = {13},
  number = {11},
  pages = {113021},
  author = {M Colom{\'{e}}-Tatch{\'{e}} and C Klempt and L Santos and T Vekua},
  title = {Adiabatic spin cooling using high-spin Fermi gases},
  journal = {New Journal of Physics}
}

%---begin---------finite-temperature Lanczos (FTL) method-------------
@article{Jakli1994,
  doi = {10.1103/physrevb.49.5065},
  url = {https://doi.org/10.1103/physrevb.49.5065},
  year = {1994},
  month = feb,
  publisher = {American Physical Society ({APS})},
  volume = {49},
  number = {7},
  pages = {5065--5068},
  author = {J. Jakli{\v{c}} and P. Prelov{\v{s}}ek},
  title = {Lanczos method for the calculation of finite-temperature quantities in correlated systems},
  journal = {Physical Review B}
}
@incollection{Prelovek2013,
  doi = {10.1007/978-3-642-35106-8_1},
  url = {https://doi.org/10.1007/978-3-642-35106-8_1},
  year = {2013},
  publisher = {Springer Berlin Heidelberg},
  pages = {1--30},
  author = {P. Prelov{\v{s}}ek and J. Bon{\v{c}}a},
  title = {Ground State and Finite Temperature Lanczos Methods},
  booktitle = {Springer Series in Solid-State Sciences}
}
%----end----------finite-temperature Lanczos (FTL) method-------------

@article{Zhang2006,
  doi = {10.1088/0305-4470/39/26/017},
  url = {https://doi.org/10.1088/0305-4470/39/26/017},
  year = {2006},
  month = jun,
  publisher = {{IOP} Publishing},
  volume = {39},
  number = {26},
  pages = {8515--8526},
  author = {Guang-Ming Zhang and Xiaoguang Wang},
  title = {Spin swapping operator as an entanglement witness for quantum Heisenberg spin-$\less$i$\greater$s$\less$/i$\greater$systems},
  journal = {Journal of Physics A: Mathematical and General}
}

@article{Beach2009,
  doi = {10.1103/physrevb.80.184401},
  url = {https://doi.org/10.1103/physrevb.80.184401},
  year = {2009},
  month = nov,
  publisher = {American Physical Society ({APS})},
  volume = {80},
  number = {18},
  pages = {184401},
  author = {K. S. D. Beach and Fabien Alet and Matthieu Mambrini and Sylvain Capponi},
  title = {$\less$mml:math xmlns:mml="http://www.w3.org/1998/Math/{MathML}" display="inline"$\greater$$\less$mml:mrow$\greater$$\less$mml:mtext$\greater${SU}$\less$/mml:mtext$\greater$$\less$mml:mrow$\greater$$\less$mml:mo$\greater$($\less$/mml:mo$\greater$$\less$mml:mi$\greater$N$\less$/mml:mi$\greater$$\less$mml:mo$\greater$)$\less$/mml:mo$\greater$$\less$/mml:mrow$\greater$$\less$/mml:mrow$\greater$$\less$/mml:math$\greater$Heisenberg model on the square lattice: A continuous-$\less$mml:math xmlns:mml="http://www.w3.org/1998/Math/{MathML}" display="inline"$\greater$$\less$mml:mi$\greater$N$\less$/mml:mi$\greater$$\less$/mml:math$\greater$quantum Monte Carlo study},
  journal = {Physical Review B}
}

@article{Ozawa2018,
  doi = {10.1103/physrevlett.121.225303},
  url = {https://doi.org/10.1103/physrevlett.121.225303},
  year = {2018},
  month = nov,
  publisher = {American Physical Society ({APS})},
  volume = {121},
  number = {22},
  pages = {225303},
  author = {Hideki Ozawa and Shintaro Taie and Yosuke Takasu and Yoshiro Takahashi},
  title = {Antiferromagnetic Spin Correlation of 
		$\less$mml:math xmlns:mml="http://www.w3.org/1998/Math/{MathML}" display="inline"$\greater$$\less$mml:mrow$\greater$$\less$mml:mi$\greater${SU}$\less$/mml:mi$\greater$$\less$mml:mo stretchy="false"$\greater$($\less$/mml:mo$\greater$$\less$mml:mi mathvariant="script"$\greater$N$\less$/mml:mi$\greater$$\less$mml:mo stretchy="false"$\greater$)$\less$/mml:mo$\greater$$\less$/mml:mrow$\greater$$\less$/mml:math$\greater$
		 Fermi Gas in an Optical Superlattice},
  journal = {Physical Review Letters}
}

@article{Taie2010,
  doi = {10.1103/physrevlett.105.190401},
  url = {https://doi.org/10.1103/physrevlett.105.190401},
  year = {2010},
  month = nov,
  publisher = {American Physical Society ({APS})},
  volume = {105},
  number = {19},
  pages = {190401},
  author = {Shintaro Taie and Yosuke Takasu and Seiji Sugawa and Rekishu Yamazaki and Takuya Tsujimoto and Ryo Murakami and Yoshiro Takahashi},
  title = {Realization of a$\less$mml:math xmlns:mml="http://www.w3.org/1998/Math/{MathML}" display="inline"$\greater$$\less$mml:mi$\greater${SU}$\less$/mml:mi$\greater$$\less$mml:mo stretchy="false"$\greater$($\less$/mml:mo$\greater$$\less$mml:mn$\greater$2$\less$/mml:mn$\greater$$\less$mml:mo stretchy="false"$\greater$)$\less$/mml:mo$\greater$$\less$mml:mo$\greater${\texttimes}$\less$/mml:mo$\greater$$\less$mml:mi$\greater${SU}$\less$/mml:mi$\greater$$\less$mml:mo stretchy="false"$\greater$($\less$/mml:mo$\greater$$\less$mml:mn$\greater$6$\less$/mml:mn$\greater$$\less$mml:mo stretchy="false"$\greater$)$\less$/mml:mo$\greater$$\less$/mml:math$\greater$System of Fermions in a Cold Atomic Gas},
  journal = {Physical Review Letters}
}

@article{Nakatsuji2005,
  doi = {10.1126/science.1114727},
  url = {https://doi.org/10.1126/science.1114727},
  year = {2005},
  month = sep,
  publisher = {American Association for the Advancement of Science ({AAAS})},
  volume = {309},
  number = {5741},
  pages = {1697--1700},
  author = {Satoru Nakatsuji and Yusuke Nambu and Hiroshi Tonomura and Osamu Sakai and Seth Jonas and Collin Broholm and Hirokazu Tsunetsugu and Yiming Qiu and Yoshiteru Maeno},
  title = {Spin Disorder on a Triangular Lattice},
  journal = {Science}
}

@article{Tsunetsugu2006,
  doi = {10.1143/jpsj.75.083701},
  url = {https://doi.org/10.1143/jpsj.75.083701},
  year = {2006},
  month = aug,
  publisher = {Physical Society of Japan},
  volume = {75},
  number = {8},
  pages = {083701},
  author = {Hirokazu Tsunetsugu and Mitsuhiro Arikawa},
  title = {Spin Nematic Phase in $\less$i$\greater$S$\less$/i$\greater$=1 Triangular Antiferromagnets},
  journal = {Journal of the Physical Society of Japan}
}
@article{Bhattacharjee2006,
  doi = {10.1103/physrevb.74.092406},
  url = {https://doi.org/10.1103/physrevb.74.092406},
  year = {2006},
  month = sep,
  publisher = {American Physical Society ({APS})},
  volume = {74},
  number = {9},
  pages = {092406},
  author = {Subhro Bhattacharjee and Vijay B. Shenoy and T. Senthil},
  title = {Possible ferro-spin nematic order in$\less$mml:math xmlns:mml="http://www.w3.org/1998/Math/{MathML}" display="inline"$\greater$$\less$mml:mrow$\greater$$\less$mml:mi mathvariant="normal"$\greater$Ni$\less$/mml:mi$\greater$$\less$mml:msub$\greater$$\less$mml:mi mathvariant="normal"$\greater$Ga$\less$/mml:mi$\greater$$\less$mml:mn$\greater$2$\less$/mml:mn$\greater$$\less$/mml:msub$\greater$$\less$mml:msub$\greater$$\less$mml:mi mathvariant="normal"$\greater$S$\less$/mml:mi$\greater$$\less$mml:mn$\greater$4$\less$/mml:mn$\greater$$\less$/mml:msub$\greater$$\less$/mml:mrow$\greater$$\less$/mml:math$\greater$},
  journal = {Physical Review B}
}
@article{Tokura2000,
  doi = {10.1126/science.288.5465.462},
  url = {https://doi.org/10.1126/science.288.5465.462},
  year = {2000},
  month = apr,
  publisher = {American Association for the Advancement of Science ({AAAS})},
  volume = {288},
  number = {5465},
  pages = {462--468},
  author = {Y. Tokura and N. Nagaosa},
  title = {Orbital Physics in Transition-Metal Oxides},
  journal = {Science}
}
@article{Goerbig2011,
  doi = {10.1103/revmodphys.83.1193},
  url = {https://doi.org/10.1103/revmodphys.83.1193},
  year = {2011},
  month = nov,
  publisher = {American Physical Society ({APS})},
  volume = {83},
  number = {4},
  pages = {1193--1243},
  author = {M. O. Goerbig},
  title = {Electronic properties of graphene in a strong magnetic field},
  journal = {Reviews of Modern Physics}
}


